Sensitivities for coherent elastic scattering of solar and supernova neutrinos with future NaI(Tl) dark matter search detectors of COSINE-200/1T

We investigate the prospects for measuring the coherent elastic neutrino-nucleus scattering of solar and supernova neutrinos in future NaI(Tl) dark matter detection experiments. Considering the reduced background and improved light yield of the recently developed NaI(Tl) crystals, more than 3$\sigma$ observation sensitivities of the supernova neutrino within the Milky Way are demonstrated. In the case of the solar neutrino, approximately 3 observations are marginal with a 1 ton NaI(Tl) experiment assuming an order of magnitude reduced background, five photoelectron thresholds, and 5-year data exposure.

==> Makefile <==
main:
	pdflatex NaI_CENNS_solar_supernovae

full:
	pdflatex NaI_CENNS_solar_supernovae
	bibtex NaI_CENNS_solar_supernovae
	pdflatex NaI_CENNS_solar_supernovae
	pdflatex NaI_CENNS_solar_supernovae

submit:
	sed -f submit.sed < NaI_CENNS_solar_supernovae.tex > NaI_CENNS_solar_supernovae_submit.tex
	pdflatex NaI_CENNS_solar_supernovae_submit
	pdflatex NaI_CENNS_solar_supernovae_submit

clean:
	rm *-converted-to.pdf *.aux *.bbl *.blg *.dvi *.log *.toc *.lof *.lot *.out *~ \#*\# *Notes.bib 

